Animating an Autonomous 3D Talking Avatar

One of the main challenges with embodying a conversational agent is annotating how and when motions can be played and composed together in real-time, without any visual artifact. The inherent problem is to do so---for a large amount of motions---without introducing mistakes in the annotation. To our knowledge, there is no automatic method that can process animations and automatically label actions and compatibility between them. In practice, a state machine, where clips are the actions, is created manually by setting connections between the states with the timing parameters for these connections. Authoring this state machine for a large amount of motions leads to a visual overflow, and increases the amount of possible mistakes. In consequence, conversational agent embodiments are left with little variations and quickly become repetitive. In this paper, we address this problem with a compact taxonomy of chit chat behaviors, that we can utilize to simplify and partially automate the graph authoring process. We measured the time required to label actions of an embodiment using our simple interface, compared to the standard state machine interface in Unreal Engine, and found that our approach is 7 times faster. We believe that our labeling approach could be a path to automated labeling: once a sub-set of motions are labeled (using our interface), we could learn a prediction that could attribute a label to new clips---allowing to really scale up virtual agent embodiments.

==> Author/Commands.tex <==
%% =========================================================================================
%% Misc

%% Replace the '??' for missing references with the text 'Missing Reference' in red
\makeatletter
\def\@setref#1#2#3{%
	\ifx#1\relax
	\protect\G@refundefinedtrue
	\nfss@text{\reset@font\bfseries\textcolor{red}{Missing Reference}}%
	\@latex@warning{Reference `#3' on page \thepage \space
		undefined}%
	\else
	\expandafter#2#1\null
	\fi
}
\makeatother

%% Replace the '?' for missing citation with the text 'Missing Citation' in red
\makeatletter
\def\@citex[#1]#2{\leavevmode
	\let\@citea\@empty
	\@cite{\@for\@citeb:=#2\do
		{\@citea\def\@citea{,\penalty\@m\ }%
			\edef\@citeb{\expandafter\@firstofone\@citeb\@empty}%
			\if@filesw\immediate\write\@auxout{\string\citation{\@citeb}}\fi
			\@ifundefined{b@\@citeb}{\hbox{\reset@font\bfseries\textcolor{red}{Missing Citation}}%
				\G@refundefinedtrue
				\@latex@warning
				{Citation `\@citeb' on page \thepage \space undefined}}%
			{\@cite@ofmt{\csname b@\@citeb\endcsname}}}}{#1}}
\makeatother


%& Highlighting for later edit
\newcommand{\TODO}[1]{{\color{red}{\bfseries TODO: #1}}}
\newcommand{\fix}[1]{{\color{red}{\bfseries #1}}}
\newcommand{\review}[1]{{\color{orange}{\bfseries #1}}}
\newcommand{\note}[1]{{\color{cyan}{\bfseries #1}}}

%% References
\newcommand{\chpref}[1]{\hyperref[#1]{Chapter~\ref{#1}}}
\newcommand{\secref}[1]{\hyperref[#1]{Section~\ref{#1}}}
\newcommand{\equref}[1]{\hyperref[#1]{\eqref{#1}}}
\newcommand{\figref}[1]{\hyperref[#1]{Figure~\ref{#1}}}
\newcommand{\tabref}[1]{\hyperref[#1]{Table~\ref{#1}}}
\renewcommand{\algref}[1]{\hyperref[#1]{Algorithm~\ref{#1}}}
\newcommand{\apxref}[1]{\hyperref[#1]{Appendix~\ref{#1}}}

%% =========================================================================================
%% Mathematical functions

%% Norms
\newcommand{\norm}[1]{\pnorm{#1}{2}}
\newcommand{\normSq}[1]{\pnormSq{#1}{2}}
\newcommand{\pnorm}[2]{\| #1 \|_{#2}}
\newcommand{\pnormSq}[2]{\| #1 \|_{#2}^{2}}

%% normalize: x/||x||
\newcommand{\normalize}[1]{\frac{#1}{\norm{#1}}}

%% mean: 1/n sum(x_i)
\newcommand{\mean}[2][n]{\frac{1}{#1} \sum_{i = 0}^{#1} #2_{i}}

%% standard deviation: sqrt( 1/n sum( (x_i - y)^2 ) )
\newcommand{\std}[2]{\sqrt{\frac{1}{n} \sum_{i = 0}^{n} (#1_{i} - #2)^2}}

%% rounding
\newcommand{\floor}[1]{\left \lfloor{#1}\right \rfloor}
\newcommand{\ceil}[1]{\left \lceil{#1}\right \rceilloor}

%% =========================================================================================
%% mathematical entities

\newcommand{\vect}[1]{\mathbf{#1}}
\newcommand{\mat}[1]{\mathbf{#1}}
\newcommand{\quaternion}{\vect{q}}

\newcommand{\crossTwo}[2]{#1 \cross #2}

%% =========================================================================================
%% Physics symbols

\newcommand{\pos}{\vect{p}}
%\newcommand{\posMean}{\vect{\bar{p}}}
\newcommand{\vel}{\vect{v}}
\newcommand{\angVel}{\boldsymbol{\omega}}
\newcommand{\gravity}{\vect{g}}
\newcommand{\force}{\vect{F}}
\newcommand{\torque}{\boldsymbol{\tau}}
\newcommand{\rvec}{\vect{r}}
\newcommand{\momentum}{\mat{M}}

%% =========================================================================================
%% layers etc.

%\newcommand{\addOp}{\odot} % dot with circle
\newcommand{\addOp}{\oplus} % plus with circle


%\newcommand{\pose}{Q}
\newcommand{\pose}[1][]{\ifthenelse{\equal{#1}{}}{Q}{Q_{#1}}}

\newcommand{\headIndex}{h}
\newcommand{\bodyIndex}{b}
\newcommand{\armsIndex}{a}

\newcommand{\basePose}{\pose[Base]}

\newcommand{\additivePose}[1]{\widetilde{\pose}_{#1}}
\newcommand{\additiveHead}{\additivePose{\headIndex}}
\newcommand{\additiveBody}{\additivePose{\bodyIndex}}
\newcommand{\additiveArms}{\additivePose{\armsIndex}}

\newcommand{\additiveWeight}[1]{\omega_{#1}}
\newcommand{\additiveWeightHead}{\additiveWeight{\headIndex}}
\newcommand{\additiveWeightBody}{\additiveWeight{\bodyIndex}}
\newcommand{\additiveWeightArms}{\additiveWeight{\armsIndex}}

\newcommand{\finalHeadPose}{\pose[Head]}
\newcommand{\finalSpinePose}{\pose[Spine]}
\newcommand{\finalLegsPose}{\pose[Legs]}
\newcommand{\finalArmsPose}{\pose[Arms]}

%% =========================================================================================

%%% My commands
%\newcommand{\addtag}{\refstepcounter{equation}\tag{\theequation}}




%
%\newcommand{\simMotion}[2][]{
%	\ifthenelse{\isempty{#1}}%
%	{{#2}_{sim}} % if #1 is empty
%	{{#2}_{#1, sim}} % if #1 is not empty
%}
%\newcommand{\refMotion}[2][]{
%	\ifthenelse{\isempty{#1}}%
%	{{#2}_{ref}} % if #1 is empty
%	{{#2}_{#1, ref}} % if #1 is not empty
%}




%% Phyicsics symbols


%%% Layout
%\makeatletter
%\newcommand{\thickhline}{%
%	\noalign {\ifnum 0=`}\fi \hrule height 1pt
%	\futurelet \reserved@a \@xhline
%}
%\newcolumntype{"}{!{\vrule width 1pt}}
%\makeatother







